Solving Price Per Unit Problem Around the World: Formulating Fact Extraction as Question Answering

Price Per Unit (PPU) is an essential information for consumers shopping on e-commerce websites when comparing products. Finding total quantity in a product is required for computing PPU, which is not always provided by the sellers. To predict total quantity, all relevant quantities given in a product attributes such as title, description and image need to be inferred correctly. We formulate this problem as a question-answering (QA) task rather than named entity recognition (NER) task for fact extraction. In our QA approach, we first predict the unit of measure (UoM) type (e.g., volume, weight or count), that formulates the desired question (e.g., "What is the total volume?") and then use this question to find all the relevant answers. Our model architecture consists of two subnetworks for the two subtasks: a classifier to predict UoM type (or the question) and an extractor to extract the relevant quantities. We use a deep character-level CNN architecture for both subtasks, which enables (1) easy expansion to new stores with similar alphabets, (2) multi-span answering due to its span-image architecture and (3) easy deployment by keeping model-inference latency low. Our QA approach outperforms rule-based methods by 34.4% in precision and also BERT-based fact extraction approach in all stores globally, with largest precision lift of 10.6% in the US store.

==> sections/expansion.tex <==
We initially implemented the model architecture for US store. With the success of this launch, we tested the model for other stores such Europe (EU-5) and India (IN).

\subsection{Vocabulary Size}

Since our model architecture is character-based, we can easily test on five European countries (EU-5), namely, France, Spain, Italy, Germany, United Kingdom, thanks to character overlap in the alphabets. However, there are special characters in EU languages which do not exist in English alphabet such as \c{c}, \'{e}, \~{n}. Hence, we expanded our character list size from 99 to 128 by including the most common special characters in EU languages.

\subsection{UoM Imbalance and Categorical Attributes}
\label{categories}
Unlike US where the PPU model performs equally well on all UoM types, for IN there is a discernible imbalance across types where precision on \emph{count} type is particularly low despite the largest share in the training dataset. To quantify the imbalance, we handpicked a set of tokens that can heavily bias the model for UoM classification, especially in the initial learning stages. Let $Tok_w$ $=$ \{\emph{gm, kg, gram, grm, kilogram, ounce,...}\} be a set of \emph{weight} related tokens and $Tok_v$ $=$ \{\emph{fluid, ml, fl oz, millilitre, l, ltr, litre,...}\} for \emph{volume}. For a product, with set of words in title as $T$ and UoM type $k$, we can define $ambiguity$ for UoM classification task as follows:
\[
 Ambiguity(T,k)= 
\begin{cases}
 1,& \text{if } (T \cap Tok_w) \neq \phi \text{ \& } (k = \text{\emph{volume}})\\
 1,& \text{if } (T \cap Tok_v) \neq \phi \text{ \& } (k = \text{\emph{weight}})\\
 1,& \text{if } (T \cap (Tok_w \cup Tok_v)) \neq \phi \text{ \& } (k = \text{\emph{count}})\\
 0,& \text{otherwise}
\end{cases}
\]

Similarly, we can define ambiguity for quantity extraction task we are unable to find qualified spans from candidate quantities. Using these definitions we found that \emph{count} is most ambiguous type for both tasks, with almost three times as many ambiguous titles as \emph{weight} and \emph{volume}. Of the prominent product categories \emph{Beauty, Health} and \emph{Grocery}, \emph{Beauty} has the most ambiguous titles in count type, while \emph{Health} has the least. Overall, ambiguous titles constituted $21\%$ of our training dataset which we call \emph{hard examples}. Although this is not the only type of ambiguity for these tasks, knowing this distribution helped in adopting new training strategies. Upsampling hard examples in the training batch helped in increasing recall for \emph{weight} and \emph{volume} types by $4\%$ across \emph{product categories}. Another strategy is to use categorical attributes to train for the UoM classification task.

For the classification task we realised that the category of the product is an essential attribute to handle ambiguity in the text. While product categories themselves are generally less informative, there are interesting patterns in more granular categories like \emph{browse nodes}\footnote{A node in a browse tree. Browse trees map product categories into subcategories and lists.} and 
\emph{sub-categories}\footnote{Sub-categories associated with browse nodes.}. For instance, for \emph{browse node} \emph{Blushes} in \emph{Beauty} product-category, majority products are count type yet the model mis-predicts on most of them due to inaccurate signals from text. We modified US model architecture to handle categorical attributes, trained categorical embeddings and concatenated them to the fully connected layer in the UoM Classification network. This model performed the best among all models and also generalised better on the classification task (see Table \ref{ablation}). Specifically for \emph{Blushes}, mis-prediction rate dropped by over $60\%$ on count type.


